Retrieve Only Relevant Tables Whether Few or Many: Adaptive Table Retrieval Method

Retrieving relevant tables from extensive databases for a given natural language query is essential for accurately answering questions in tasks such as text-to-SQL. Existing table retrieval approaches select a pre-determined set of k tables with the highest similarity to the query. However, the number of required tables varies across queries and cannot be known in advance. Enforcing a fixed number of retrieved tables regardless of the query may either retrieve an undersized set, failing to obtain all necessary evidence, or retrieve an oversized pool, including irrelevant tables. To address this issue, we propose an adaptive table retrieval method that adjusts the number of tables retrieved according to the requirements of each query. Specifically, we utilize an adaptive thresholding mechanism to selectively retrieve tables and integrate a sliding-window reranking algorithm to efficiently process a large table corpus. Extensive experiments on Spider, BIRD, and Spider 2.0 demonstrate that our method effectively addresses the limitations of the top-k retrieval strategy, improving performance in retrieval and downstream tasks. Our code and data are available at https://github.com/sbY99/Adaptive-Table-Retrieval.

==> latex/tables/_end-to-end_performance.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
                                             &            & \multicolumn{2}{c}{\textbf{Spider}}                                                                                                  & \multicolumn{2}{c}{\textbf{BIRD}}                                                                                                    & \multicolumn{2}{c}{\textbf{Spider 2.0}}                                                                                              \\ \cline{2-8} 
                                             & \textit{k} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} \\ \hline
\multicolumn{8}{l}{\textit{\textbf{Encoder-based}}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
Contriever                                   & 3          & 54.6 / 64.8                                                       & 65.4 / 66.3                                                      & 21.7 / 40.4                                                       & 35.4 / 46.0                                                      & \underline{1.1} / 3.4                                                         & 0.5 / 3.9                                                        \\
                                             & 5          & 53.3 / 65.0                                                       & 65.7 / 68.6                                                      & 22.4 / 44.5                                                       & 37.0 / 49.8                                                      & \underline{1.1} / 3.2                                                         & 1.4 / 3.7                                                        \\
                                             & 10         & 54.6 / 67.1                                                       & 66.0 / 70.1                                                      & 24.3 / 47.4                                                       & 39.1 / 53.0                                                      & \underline{1.1} / 3.5                                                         & 0.9 / 4.1                                                        \\
UAE                                          & 3          & 55.7 / 65.0                                                       & 63.6 / 68.0                                                      & 22.6 / 40.7                                                       & 35.1 / 45.4                                                      & 0.7 / 3.5                                                         & 1.1 / 3.4                                                        \\
                                             & 5          & 54.9 / 66.1                                                       & 66.0 / 69.6                                                      & 23.9 / 45.0                                                       & 37.8 / 49.5                                                      & 0.9/ 3.9                                                          & 1.1 / 3.4                                                        \\
                                             & 10         & 54.7 / 67.3                                                       & 66.1 / 70.6                                                      & 26.0 / 47.9                                                       & 40.4 / 52.2                                                      & 1.4/ 4.1                                                          & 1.4 / 3.4                                                        \\ \hline
\multicolumn{8}{l}{\textit{\textbf{LLM-based}}}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
RankZephyr                                   & 3          & 53.3  / 64.8                                                      & 63.1 / 66.6                                                      & 22.4 / 40.7                                                       & 34.5 / 45.8                                                      & \underline{1.1} / 3.2                                                         & 1.4 / 4.1                                                        \\
                                             & 5          & 54.8 / 65.9                                                       & 65.4 / 67.2                                                      & 23.0 / 45.0                                                       & 38.1 / 46.2                                                      & 0.9 / 3.0                                                         & 1.1 / 4.1                                                        \\
                                             & 10         & 57.5 / 67.0                                                       & 66.4 / 67.3                                                      & 25.4 / 47.5                                                       & 39.3 / 49.5                                                      & \underline{1.1} / 3.4                                                         & 1.4 / 3.4                                                        \\
Murre                              & 3          & 51.2 / 65.3                                                       & 63.4 / 64.6                                                      & 21.8 / 44.5                                                       & 34.2 / 44.2                                                      & 0.9 / 4.1                                                         & 1.4 / 3.2                                                        \\
                                             & 5          & 53.7 / 65.6                                                       & 64.1 / 65.8                                                      & 22.6 / 44.8                                                       & 37.5 / 45.4                                                      & 0.9 / 3.0                                                         & 1.4 / 3.7                                                        \\
                                             & 10         & 54.5 / 65.9                                                       & 65.3 / 68.0                                                      & 25.3 / 46.4                                                       & 39.4 / 48.4                                                      & 0.7 / 4.1                                                         & 1.4 / 4.4                                                        \\ \hline
\multicolumn{8}{l}{\textit{\textbf{Reranker-based}}}                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
% BGE-M3 + Contriever                          & 3          & 53.1 / 65.9                                                       & 64.8 / 64.9                                                      & 20.5 / 36.6                                                       & 31.2 / 36.1                                                      & 0.5 / 2.5                                                         & 0.2 / 2.3                                                        \\
%                                              & 5          & 55.0 / 66.4                                                       & 66.2 / 66.7                                                      & 22.1 / 42.1                                                       & 33.5 / 41.1                                                      & 0.9 / 3.4                                                         & 0.5 / 2.8                                                        \\
%                                              & 10         & 54.3 / 65.2                                                       & 65.8 / 66.1                                                      & 24.1 / 45.2                                                       & 36.6 / 44.9                                                      & 0.9 / 3.9                                                         & 0.5 / 3.4                                                        \\
% BGE-M3 + UAE                                 & 3          & 52.4 / 65.7                                                       & 65.4 / 66.3                                                      & 19.6 / 34.6                                                       & 28.2 / 37.8                                                      & 0.7 / 3.4                                                         & 0.9 / 2.3                                                        \\
%                                              & 5          & 54.9 / 66.3                                                       & 67.1 / 68.5                                                      & 22.2 / 40.6                                                       & 33.3 / 44.7                                                      & 0.9 / 3.7                                                         & 1.1 / 3.4                                                        \\
%                                              & 10         & 53.9 / 65.2                                                       & 66.5 / 69.4                                                      & 25.0 / 44.3                                                       & 36.6 / 49.8                                                      & \underline{1.1} / 3.7                                                         & 0.5 / 3.4                                                        \\
JAR (w. Contriever)                             & 3          & 53.9 / 65.9                                                       & 66.6 / 68.8                                                      & 25.4 / 45.3                                                       & 40.1 / 49.7                                                      & 0.7 / 3.7                                                         & 0.9 / 4.1                                                        \\
                                             & 5          & 54.8 / 66.6                                                       & 67.5 / 69.7                                                      & 26.8 / 46.4                                                       & 43.4 / 52.0                                                      & \underline{1.1} / 3.9                                                   & 0.7 / 3.7                                                        \\
                                             & 10         & 56.0 / 66.8                                                       & 66.6 / 69.2                                                      & 26.7 / 47.5                                                       & 43.0 / 53.0                                                      & 0.9 / 3.0                                                         & 1.4 / 4.4                                                        \\
JAR (w. UAE)                                    & 3          & 54.6 / 67.2                                                       & 66.7 / 66.8                                                      & 24.8 / 44.7                                                       & 38.7 / 44.9                                                      & 0.9 / 3.9                                                         & \underline{1.6} / 4.4                                                  \\
                                             & 5          & 56.0 / 67.4                                                       & 67.0 / 69.7                                                      & 25.3 / 45.4                                                       & 39.2 / 48.4                                                      & 0.9 / 4.1                                                         & 1.4 / 4.1                                                        \\
                                             & 10         & 55.6 / 66.9                                                       & 64.6 / 67.7                                                      & 26.6 / 46.9                                                       & 41.3 / 52.2                                                      & 0.9 / 3.0                                                         & \underline{1.6} / 3.7                                                  \\ \bottomrule
\multicolumn{8}{l}{\textit{\textbf{Ours}}}                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
ATR (w. Contriever)                             &            & \underline{58.7} / \underline{67.8}                                                 & \underline{69.7} / \textbf{71.5}                                                & \underline{28.6} / \textbf{49.9}                                                 & \textbf{45.0} / \underline{53.3}                                             & \underline{1.1} / \underline{4.4}                                                   & 1.4 / \textbf{5.7}                                               \\
ATR (w. UAE)                                    &            & \textbf{59.8} / \textbf{68.2}                                              & \textbf{69.8} / \underline{71.4}                                             & \textbf{29.0} / \underline{48.7}                                              & \underline{43.8} / \textbf{53.9}                                                & \textbf{1.6 / 4.5}                                                & \textbf{2.1} / \underline{4.9}                                               \\ \bottomrule
\multicolumn{1}{l}{\textit{\textbf{Oracle}}} &            & 66.6 / 70.8                                                       & 75.6 / 75.2                                                      & 31.8 / 53.5                                                       & 50.6 / 58.0                                                      & 4.4 / 7.2                                                         & 3.5 / 7.4                       \\ \bottomrule                               
\end{tabular}%
}
\caption{Text-to-SQL execution accuracy comparison across different table retrieval methods. ATR consistently outperforms baseline retrievers on the Spider, BIRD, and Spider 2.0 datasets.}
\label{tab:end-to-end_performance_}
\end{table*}

==> latex/tables/sliding_analysis.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{cccccccccc}
\hline
                                                                               & \multicolumn{3}{c}{\textbf{Spider}} & \multicolumn{3}{c}{\textbf{BIRD}} & \multicolumn{3}{c}{\textbf{Spider 2.0}} \\ \hline
\textbf{W, R} & 50, N/A     & 20, 15     & 10, 6    & 50, N/A    & 20, 15     & 10,6    & 50, N/A       & 10, 5      & 6, 4       \\ \hline
\textbf{Time}                                                           & 0.12        & 0.14       & 0.17     & 0.18       & 0.21       & 0.26    & 0.60          & 0.41       & 0.45       \\
\textbf{Length}                                                                  & 1164.4      & 471.7      & 237.5    & 1592.7     & 617.9      & 324.0   & 3982.8        & 846.2      & 532.8      \\
\textbf{\# Inference}                                                          & 1           & 7          & 11       & 1          & 7    & 11      & 1             & 9          & 23         \\ \hline
\end{tabular}
\caption{Analysis of sliding window hyper-parameters $W$ and $R$, where $W$ denotes the window size and $R$ is the retention size. The metrics include average inference time in seconds (Time), average input token length (Length), and number of inferences (\# Inference).}
\label{tab:sliding analysis}
\end{table*}

==> tables/_end-to-end_performance.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
                                             &            & \multicolumn{2}{c}{\textbf{Spider}}                                                                                                  & \multicolumn{2}{c}{\textbf{BIRD}}                                                                                                    & \multicolumn{2}{c}{\textbf{Spider 2.0}}                                                                                              \\ \cline{2-8} 
                                             & \textit{k} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} \\ \hline
\multicolumn{8}{l}{\textit{\textbf{Encoder-based}}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
Contriever                                   & 3          & 54.6 / 64.8                                                       & 65.4 / 66.3                                                      & 21.7 / 40.4                                                       & 35.4 / 46.0                                                      & \underline{1.1} / 3.4                                                         & 0.5 / 3.9                                                        \\
                                             & 5          & 53.3 / 65.0                                                       & 65.7 / 68.6                                                      & 22.4 / 44.5                                                       & 37.0 / 49.8                                                      & \underline{1.1} / 3.2                                                         & 1.4 / 3.7                                                        \\
                                             & 10         & 54.6 / 67.1                                                       & 66.0 / 70.1                                                      & 24.3 / 47.4                                                       & 39.1 / 53.0                                                      & \underline{1.1} / 3.5                                                         & 0.9 / 4.1                                                        \\
UAE                                          & 3          & 55.7 / 65.0                                                       & 63.6 / 68.0                                                      & 22.6 / 40.7                                                       & 35.1 / 45.4                                                      & 0.7 / 3.5                                                         & 1.1 / 3.4                                                        \\
                                             & 5          & 54.9 / 66.1                                                       & 66.0 / 69.6                                                      & 23.9 / 45.0                                                       & 37.8 / 49.5                                                      & 0.9/ 3.9                                                          & 1.1 / 3.4                                                        \\
                                             & 10         & 54.7 / 67.3                                                       & 66.1 / 70.6                                                      & 26.0 / 47.9                                                       & 40.4 / 52.2                                                      & 1.4/ 4.1                                                          & 1.4 / 3.4                                                        \\ \hline
\multicolumn{8}{l}{\textit{\textbf{LLM-based}}}                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
RankZephyr                                   & 3          & 53.3  / 64.8                                                      & 63.1 / 66.6                                                      & 22.4 / 40.7                                                       & 34.5 / 45.8                                                      & \underline{1.1} / 3.2                                                         & 1.4 / 4.1                                                        \\
                                             & 5          & 54.8 / 65.9                                                       & 65.4 / 67.2                                                      & 23.0 / 45.0                                                       & 38.1 / 46.2                                                      & 0.9 / 3.0                                                         & 1.1 / 4.1                                                        \\
                                             & 10         & 57.5 / 67.0                                                       & 66.4 / 67.3                                                      & 25.4 / 47.5                                                       & 39.3 / 49.5                                                      & \underline{1.1} / 3.4                                                         & 1.4 / 3.4                                                        \\
Murre                              & 3          & 51.2 / 65.3                                                       & 63.4 / 64.6                                                      & 21.8 / 44.5                                                       & 34.2 / 44.2                                                      & 0.9 / 4.1                                                         & 1.4 / 3.2                                                        \\
                                             & 5          & 53.7 / 65.6                                                       & 64.1 / 65.8                                                      & 22.6 / 44.8                                                       & 37.5 / 45.4                                                      & 0.9 / 3.0                                                         & 1.4 / 3.7                                                        \\
                                             & 10         & 54.5 / 65.9                                                       & 65.3 / 68.0                                                      & 25.3 / 46.4                                                       & 39.4 / 48.4                                                      & 0.7 / 4.1                                                         & 1.4 / 4.4                                                        \\ \hline
\multicolumn{8}{l}{\textit{\textbf{Reranker-based}}}                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
% BGE-M3 + Contriever                          & 3          & 53.1 / 65.9                                                       & 64.8 / 64.9                                                      & 20.5 / 36.6                                                       & 31.2 / 36.1                                                      & 0.5 / 2.5                                                         & 0.2 / 2.3                                                        \\
%                                              & 5          & 55.0 / 66.4                                                       & 66.2 / 66.7                                                      & 22.1 / 42.1                                                       & 33.5 / 41.1                                                      & 0.9 / 3.4                                                         & 0.5 / 2.8                                                        \\
%                                              & 10         & 54.3 / 65.2                                                       & 65.8 / 66.1                                                      & 24.1 / 45.2                                                       & 36.6 / 44.9                                                      & 0.9 / 3.9                                                         & 0.5 / 3.4                                                        \\
% BGE-M3 + UAE                                 & 3          & 52.4 / 65.7                                                       & 65.4 / 66.3                                                      & 19.6 / 34.6                                                       & 28.2 / 37.8                                                      & 0.7 / 3.4                                                         & 0.9 / 2.3                                                        \\
%                                              & 5          & 54.9 / 66.3                                                       & 67.1 / 68.5                                                      & 22.2 / 40.6                                                       & 33.3 / 44.7                                                      & 0.9 / 3.7                                                         & 1.1 / 3.4                                                        \\
%                                              & 10         & 53.9 / 65.2                                                       & 66.5 / 69.4                                                      & 25.0 / 44.3                                                       & 36.6 / 49.8                                                      & \underline{1.1} / 3.7                                                         & 0.5 / 3.4                                                        \\
JAR (w. Contriever)                             & 3          & 53.9 / 65.9                                                       & 66.6 / 68.8                                                      & 25.4 / 45.3                                                       & 40.1 / 49.7                                                      & 0.7 / 3.7                                                         & 0.9 / 4.1                                                        \\
                                             & 5          & 54.8 / 66.6                                                       & 67.5 / 69.7                                                      & 26.8 / 46.4                                                       & 43.4 / 52.0                                                      & \underline{1.1} / 3.9                                                   & 0.7 / 3.7                                                        \\
                                             & 10         & 56.0 / 66.8                                                       & 66.6 / 69.2                                                      & 26.7 / 47.5                                                       & 43.0 / 53.0                                                      & 0.9 / 3.0                                                         & 1.4 / 4.4                                                        \\
JAR (w. UAE)                                    & 3          & 54.6 / 67.2                                                       & 66.7 / 66.8                                                      & 24.8 / 44.7                                                       & 38.7 / 44.9                                                      & 0.9 / 3.9                                                         & \underline{1.6} / 4.4                                                  \\
                                             & 5          & 56.0 / 67.4                                                       & 67.0 / 69.7                                                      & 25.3 / 45.4                                                       & 39.2 / 48.4                                                      & 0.9 / 4.1                                                         & 1.4 / 4.1                                                        \\
                                             & 10         & 55.6 / 66.9                                                       & 64.6 / 67.7                                                      & 26.6 / 46.9                                                       & 41.3 / 52.2                                                      & 0.9 / 3.0                                                         & \underline{1.6} / 3.7                                                  \\ \bottomrule
\multicolumn{8}{l}{\textit{\textbf{Ours}}}                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
ATR (w. Contriever)                             &            & \underline{58.7} / \underline{67.8}                                                 & \underline{69.7} / \textbf{71.5}                                                & \underline{28.6} / \textbf{49.9}                                                 & \textbf{45.0} / \underline{53.3}                                             & \underline{1.1} / \underline{4.4}                                                   & 1.4 / \textbf{5.7}                                               \\
ATR (w. UAE)                                    &            & \textbf{59.8} / \textbf{68.2}                                              & \textbf{69.8} / \underline{71.4}                                             & \textbf{29.0} / \underline{48.7}                                              & \underline{43.8} / \textbf{53.9}                                                & \textbf{1.6 / 4.5}                                                & \textbf{2.1} / \underline{4.9}                                               \\ \bottomrule
\multicolumn{1}{l}{\textit{\textbf{Oracle}}} &            & 66.6 / 70.8                                                       & 75.6 / 75.2                                                      & 31.8 / 53.5                                                       & 50.6 / 58.0                                                      & 4.4 / 7.2                                                         & 3.5 / 7.4                       \\ \bottomrule                               
\end{tabular}%
}
\caption{Text-to-SQL execution accuracy comparison across different table retrieval methods. ATR consistently outperforms baseline retrievers on the Spider, BIRD, and Spider 2.0 datasets.}
\label{tab:end-to-end_performance_}
\end{table*}

==> tables/ablation_study.tex <==
\begin{table}[t!]
\centering
\setlength{\tabcolsep}{1.2mm} 
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\hline
                       & \multicolumn{2}{c}{\textbf{Spider}}             & \multicolumn{2}{c}{\textbf{BIRD}}               & \multicolumn{2}{c}{\textbf{Spider 2.0}}    \\ \cline{2-7}
                       & \textbf{R}      & \textbf{CR} & \textbf{R}      & \textbf{CR} & \textbf{R} & \textbf{CR} \\ \hline
\textbf{ATR}          & { \textbf{99.5}} & { \textbf{99.2}}     & {\textbf{98.2}} & { \textbf{96.0}}     & {\textbf{72.4}}     & { \textbf{64.4}}              \\ \hline
$-$ (1) BCE         & \underline{99.0}                & \underline{98.7}              & \underline{97.5}          & \underline{95.8}              & \underline{68.2}     & \underline{60.8}              \\
$-$ (2) Contrastive & \underline{99.0}          & 98.4                    & 97.4                & 95.2                    & 69.1           & 60.1                    \\ 
$-$ (1) \& (2)        & 96.4                & 94.4                    & 91.8                & 85.7                    & 67.7                    & 58.2                    \\ 
\hline
\end{tabular}%
}
\caption{Ablation study on table representation losses.}
% \caption{Ablation study on training objectives for table representation. Both loss functions contribute significantly to the retrieval performance of ATR.}
\label{tab:ablation}
% \end{adjustbox}
\end{table}

==> tables/adaptive_retrieval_performance.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1mm} 
\begin{adjustbox}{width=1\columnwidth}
\begin{tabular}{lcccccc}
\toprule
\textbf{} & \multicolumn{3}{c}{\textbf{Spider}} & \multicolumn{3}{c}{\textbf{BIRD}} \\ \cline{2-7}

 & \textbf{R} & \textbf{Acc.} & \textbf{Time($\downarrow$)} & \textbf{R} & \textbf{Acc.} & \textbf{Time($\downarrow$)} \\ \hline
 
\textbf{{Iter-RetGen}} & \underline{98.8} & {\textbf{71.7}} & 8.9 & \underline{96.5} & \underline{52.7} & 14.4 \\

\textbf{{FLARE}} & 89.0 & 63.2 & \underline{4.0} & 78.3 & 43.1 & \underline{5.7} \\ 

\textbf{{Adaptive-RAG}} & 86.0 & 62.8 & 6.3 & 89.8 & 50.7 & 13.2 \\ 
\hline
\textbf{ATR (Ours)} & \textbf{99.5} & \underline{71.5} & \textbf{2.2} & \textbf{98.2} & \textbf{53.3} & \textbf{3.8} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{ATR outperforms existing adaptive document retrieval strategies in both efficiency and accuracy. Acc. and Time denote execution accuracy and the average end-to-end inference time in seconds, respectively.}
\label{tab:adaptive_retrieval}
\end{table}

==> tables/additional_end-to-end_performance.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lc cccc cccc cccc}
\toprule
 &  & \multicolumn{4}{c}{\textbf{Spider}} & \multicolumn{4}{c}{\textbf{BIRD}} & \multicolumn{4}{c}{\textbf{Spider 2.0}} \\ \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & \textit{k} & \textbf{Qwen3} & \textbf{DeepSeek-V2} & \textbf{GPT-5} & \textbf{Gemini-2.5} & \textbf{Qwen3} & \textbf{DeepSeek-V2} & \textbf{GPT-5} & \textbf{Gemini-2.5} & \textbf{Qwen3} & \textbf{DeepSeek-V2} & \textbf{GPT-5} & \textbf{Gemini-2.5} \\ \hline
\multicolumn{14}{l}{\textit{\textbf{Encoder-based}}} \\ \hline
Contriever & 3 & 71.7 & 61.7 & 60.4 & 73.7 & 45.2 & 29.9 & 35.1 & 48.8 & 3.2 & 1.8 & 3.2 & 2.5 \\
 & 5 & 74.2 & 61.9 & 63.4 & 75.0 & 50.3 & 32.3 & 37.5 & 54.0 & 3.2 & 1.6 & 5.1 & 3.9 \\
 & 10 & 75.9 & 62.3 & 64.8 & 76.5 & 53.7 & 36.8 & 40.4 & 58.1 & 3.7 & 1.6 & 5.8 & 4.4 \\
UAE & 3 & 71.9 & 61.5 & 60.6 & 73.3 & 46.1 & 31.8 & 34.2 & 50.5 & 3.7 & 1.6 & 4.6 & 2.5 \\
 & 5 & 75.9 & 62.4 & 64.0 & 76.3 & 49.7 & 33.6 & 37.6 & 54.8 & 3.9 & \underline{2.8} & 5.3 & 4.6 \\
 & 10 & 76.2 & 63.8 & 65.1 & 76.9 & 54.0 & 38.3 & 41.3 & 59.3 & 4.4 & 1.8 & 7.6 & 4.6 \\ \hline
\multicolumn{14}{l}{\textit{\textbf{LLM-based}}} \\ \hline
RankZephyr & 3 & 71.3 & 62.4 & 60.1 & 73.2 & 45.1 & 29.7 & 36.0 & 48.6 & 3.2 & 2.1 & 5.1 & 4.1 \\
 & 5 & 74.3 & 61.3 & 64.9 & 75.4 & 51.2 & 33.1 & 37.9 & 54.1 & 3.5 & 0.9 & 4.6 & 3.5 \\
 & 10 & 76.2 & 63.2 & 65.0 & 76.9 & \underline{54.6} & 37.0 & 40.0 & 58.7 & 3.7 & 1.8 & 7.4 & 5.1 \\
Murre & 3 & 71.3 & 62.4 & 60.7 & 73.9 & 49.3 & 30.1 & 36.1 & 50.3 & 2.5 & 2.3 & 4.1 & 3.5 \\
 & 5 & 74.1 & 63.6 & 62.8 & 74.6 & 50.5 & 32.5 & 37.0 & 52.5 & 3.9 & 2.3 & 5.8 & 5.3 \\
 & 10 & 75.9 & 64.4 & 64.3 & 76.2 & 53.6 & 37.3 & 41.3 & 58.7 & 4.1 & 2.1 & 7.4 & 5.5 \\ \hline
\multicolumn{14}{l}{\textit{\textbf{Reranker-based}}} \\ \hline
JAR  & 3 & 74.5 & 63.8 & 63.2 & 74.8 & 49.3 & 36.3 & 37.1 & 55.3 & 2.3 & 2.1 & 4.8 & 3.2 \\
(w. Contriever) & 5 & 74.6 & 61.9 & 64.5 & 76.4 & 52.4 & 37.0 & 37.7 & 56.5 & 3.0 & 1.6 & 5.3 & 4.6 \\
 & 10 & 75.6 & 63.1 & 66.2 & 76.5 & 54.0 & 38.2 & 39.4 & 58.1 & 3.9 & 2.3 & 5.5 & 4.4 \\
JAR  & 3 & 74.6 & 62.9 & 65.4 & 75.8 & 49.6 & 36.3 & 37.2 & 52.9 & 3.0 & 2.5 & 4.4 & 4.1 \\
(w. UAE) & 5 & 76.2 & 63.1 & 67.1 & 77.4 & 50.6 & 36.8 & 38.0 & 54.3 & 3.2 & 2.3 & 5.8 & 4.6 \\
 & 10 & 75.6 & 64.7 & \underline{67.3} & \underline{78.1} & 53.6 & 38.0 & 41.1 & 57.7 & 3.0 & 2.5 & 6.9 & 5.5 \\ \hline
\multicolumn{14}{l}{\textit{\textbf{Ours}}} \\ \hline
ATR &  & \underline{76.3} & \textbf{66.4} & 65.5 & 77.9 & \textbf{55.0} & \underline{38.5} & \underline{41.6} & \underline{59.4} & \underline{4.6} & \textbf{3.0} & \textbf{9.0} & \underline{5.8} \\
(w. Contriever) & & & & & & & & & & & & & \\
ATR &  & \textbf{76.7} & \underline{65.8} & \textbf{67.8} & \textbf{79.4} & 54.3 & \textbf{39.6} & \textbf{41.9} & \textbf{59.5} & \textbf{4.8} & 2.5 & \underline{8.5} & \textbf{6.7} \\ 
(w. UAE) & & & & & & & & & & & & & \\
\hline
\textit{\textbf{Oracle}} &  & 79.0 & 71.4 & 68.3 & 79.7 & 59.5 & 44.9 & 43.1 & 62.8 & 9.0 & 5.1 & 11.5 & 8.9 \\ \bottomrule
\end{tabular}%
}
\caption{Text-to-SQL execution accuracy comparison for the various models, including open source and proprietary LLMs, across different table retrieval methods.}
\label{tab:additional_end-to-end_performance}
\end{table*}

==> tables/case_study_1.tex <==
\begin{table*}[ht]
\centering
% \toprule
% \hline
\begin{tabular}{p{0.48\textwidth}p{0.48\textwidth}}
% \hline
\toprule
\multicolumn{2}{p{0.96\textwidth}}{
\textbf{Question}\vspace{2pt}} \\
% \hline
% \toprule
\bottomrule
\multicolumn{2}{p{0.96\textwidth}}{
\begin{minipage}[c]{0.96\textwidth}
\vspace{6pt}
Please list player names which are higher than 180.
\vspace{6pt}
\end{minipage}
} 
% \vspace{0.01\textheight}
\\

% \hline
\toprule
\textbf{Tables Retrieved by ATR} & \textbf{Tables Retrieved by Top-$k$} \\
% \hline
\bottomrule

\begin{minipage}[t]{0.48\textwidth}
"Player"
% ["european\_football\_2", 
% "Player"]
\end{minipage} 
&
\begin{minipage}[c]{0.48\textwidth}
\vspace{6pt}
"Player" \newline
\textcolor{red}{"Match"} \newline \textcolor{red}{"League"} \newline \textcolor{red}{"Team"} \newline  \textcolor{red}{"superhero"}
% \includegraphics[width=0.86\textwidth]
% {latex/images/case_study_ours_1.pdf}
% ["european\_football\_2", "Player"] \newline 
\vspace{6pt}
\end{minipage} \\
% \hline
\toprule
\textbf{SQL Generated by ATR} & \textbf{SQL Generated by Top-$k$} \\
% \hline
\bottomrule
\begin{minipage}[c]{0.48\textwidth}
%SELECT player\_name FROM Player WHERE height > 180 
\vspace{6pt}
\includegraphics[width=0.86\textwidth]
{latex/images/case_study_ours_1.pdf}
% "Player" \newline 
% \textcolor{red}{"Match"} \textcolor{red}{"Team"} 
% \newline
% \textcolor{red}{"League"} \textcolor{red}{"superhero"}
\vspace{6pt}
\end{minipage}
&
\begin{minipage}[c]{0.48\textwidth}
%SELECT T1.player\_name FROM Player AS T1 INNER JOIN Match
%AS T2 ON T1.player\_api\_id = T2.home\_player\_1 WHERE T1.height > %180 
\includegraphics[width=1.5\textwidth]
{latex/images/case_study_baseline_1.pdf}
\end{minipage} \\
% \hline
\toprule
\multicolumn{2}{p{0.96\textwidth}}{\textbf{Retrieved Table Schema}} \\
% \hline
\bottomrule
\multicolumn{2}{p{0.96\textwidth}}{
\begin{minipage}[c]{0.96\textwidth}
\vspace{6pt}
"Player": \textit{id}, \textit{player\_api\_id}, \textit{height}, \textit{weight}, \textit{birthday}, \textit{player\_name}, \textit{player\_fifa\_api\_id} \newline
\textcolor{red}{"Match": \textit{id}, \textit{home\_player\_1}, \textit{stage}, \textit{goal}, \textit{season}, \textit{country\_id}, \textit{league\_id}, \textit{match\_api\_id}, ...} \newline
\textcolor{red}{"League": \textit{id}, \textit{country\_id}, \textit{name} } \newline
\textcolor{red}{"Team": \textit{id}, \textit{team\_api\_id}, \textit{team\_fifa\_api\_id}, \textit{team\_long\_name}, \textit{team\_short\_name}}  \newline
\textcolor{red}{"superhero": \textit{id}, \textit{superhero\_name}, \textit{full\_name}, \textit{gender\_id}, \textit{eye\_colour\_id}, \textit{hair\_colour\_id}, ...}
% ["european\_football\_2", "Player"]|: Player.id, Player.player\_api\_id, Player.height .. \newline
% ["european\_football\_2", "Match"]: Match.home\_player\_1, Match.match\_api\_id, Match.goal, .. \newline
% ["european\_football\_2", "Team"]: Team.id, Team.team\_api\_id, ..  \newline
% ["european\_football\_2", "League"]: League.id, League.country\_id, ..  \newline
% ["superhero", "superhero"]: superhero.id, superhero.superhero\_name, superhero.height\_kg, ..
\vspace{6pt}
\end{minipage}
} \\
% \hline
\bottomrule
\end{tabular}
\caption{
A case study illustrating a scenario where the retrieval size $k$ exceeds the number of tables required to resolve the query. As the top-$k$ approach retrieves unnecessary tables, it propagates noise, degrading downstream SQL generation. Irrelevant tables are in red, and unnecessary tables that do not contribute to answering the query are highlighted in yellow. Retrieved table schema displays schema information for all retrieved tables.
% irrelevant한 table로 인해 downstream task degradation 하는 케이스
% Scenario where fixed $k$ exceeds the required number of tables. Tables retrieved by the top-$k
% $ method but irrelevant to SQL generation are indicated in red text. Text highlighted in yellow represents unnecessary tables that do not contribute to answering the question. Retrieved Table Schema displays schema information for all retrieved tables.
% Retrieved Table Schema denotes the schema information for tables retrieved by ATR and top-$k$.
} 
\label{tab: case study 1: k as noise}
\end{table*}

==> tables/case_study_2.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{p{0.48\textwidth}p{0.48\textwidth}}
% \hline
\toprule
\multicolumn{2}{p{0.96\textwidth}}{\textbf{Question}} \\
\bottomrule
% \hline
\multicolumn{2}{p{0.96\textwidth}}{
\begin{minipage}[c]{0.96\textwidth}
\vspace{6pt}
Please calculate the monthly average levels of PM10, PM2.5 FRM, PM2.5 non-FRM, volatile organic emissions, SO2 (scaled by a factor of 10), and Lead (scaled by a factor of 100) air pollutants in California for the year 2020.
\vspace{6pt}
\end{minipage}} \\
% \hline
\toprule
\textbf{Tables Retrieved by ATR} & \textbf{Tables Retrieved by Top-$k$} \\
% \hline
\bottomrule
\begin{minipage}[c]{0.48\textwidth}
\vspace{6pt}
"pm25\_frm\_daily\_summary" \newline
"lead\_daily\_summary" \newline
"pm10\_daily\_summary" \newline
"pm25\_nonfrm\_daily\_summary" \newline
"so2\_daily\_summary" \newline
"voc\_daily\_summary"
\vspace{6pt}
\end{minipage} 
&
\begin{minipage}[c]{0.48\textwidth}
\vspace{6pt}
"pm25\_frm\_daily\_summary" \newline
"lead\_daily\_summary" \newline
"pm10\_daily\_summary" \newline
\textcolor{red}{"pm25\_frm\_hourly\_summary"} \newline
\textcolor{red}{"pm10\_hourly\_summary"} \newline
\textcolor{lightgray}{"pm25\_nonfrm\_daily\_summary"} \newline
\textcolor{lightgray}{"so2\_daily\_summary"} \newline
\textcolor{lightgray}{"voc\_daily\_summary"}
\vspace{6pt}
\end{minipage} \\
% \hline
\toprule
\textbf{SQL Generated by ATR} & \textbf{SQL Generated by Top-$k$} \\
% \hline
\bottomrule
%SELECT player\_name FROM Player WHERE height > 180 
\vspace{1pt}
\includegraphics[width=0.48\textwidth]
{latex/images/case_study_ours_2.pdf}
\vspace{1pt}
&
%SELECT T1.player\_name FROM Player AS T1 INNER JOIN Match
%AS T2 ON T1.player\_api\_id = T2.home\_player\_1 WHERE T1.height > %180 
\vspace{1pt}
\includegraphics[width=0.48\textwidth]
{latex/images/case_study_baseline_2_ver2.pdf}
\vspace{1pt}\\
% \hline
\toprule
\multicolumn{2}{p{0.96\textwidth}}{\textbf{Retrieved Table Schema}} \\
% \hline
\bottomrule
\multicolumn{2}{p{0.96\textwidth}}{
\begin{minipage}[c]{0.96\textwidth}
\vspace{2pt}
"pm25\_frm\_daily\_summary": \textit{arithmetic\_mean}, \textit{date\_local}, \textit{state\_code}, \textit{county\_code}, ... \newline
"lead\_daily\_summary": \textit{arithmetic\_mean}, \textit{date\_local}, \textit{state\_code}, \textit{county\_code}, ...\newline
"pm10\_daily\_summary": \textit{arithmetic\_mean}, \textit{date\_local}, \textit{state\_code}, \textit{county\_code}, ... \newline
"pm25\_nonfrm\_daily\_summary": \textit{arithmetic\_mean}, \textit{date\_local}, \textit{state\_code}, \textit{county\_code}, ... \newline
"so2\_daily\_summary": \textit{arithmetic\_mean}, \textit{date\_local}, \textit{state\_code}, \textit{county\_code}, ... \newline
"voc\_daily\_summary": \textit{arithmetic\_mean}, \textit{date\_local}, \textit{state\_code}, \textit{county\_code}, ... \newline
\textcolor{red}{"pm25\_frm\_hourly\_summary": \textit{date\_local}, \textit{sample\_measurement}, \textit{state\_code}, \textit{county\_code},  ...} \newline
\textcolor{red}{"pm10\_hourly\_summary": \textit{date\_local}, \textit{sample\_measurement}, \textit{state\_code}, \textit{county\_code}, ...}
\vspace{2pt}
\end{minipage}
} \\
% \hline
\bottomrule
\end{tabular}
\caption{
A case study illustrating a scenario where the retrieval size $k$ is smaller than the number of tables required to resolve the query. As the top-
$k$ approach fails to retrieve all necessary tables, it produces inaccurate SQL, whereas ATR retrieves all essential tables, enabling correct SQL generation. Tables not retrieved but crucial for SQL generation are displayed in light gray.
% 필요한 table을 뽑지못해 downstream task를 수행하지 못하는 상황
% Scenario where more tables are needed than the fixed $k$. Neccessary but not retrieved by the top-$k$ method are not marked in lightgray text.
% Unnecessary tables retrieved by the top-$k$ method are marked in red text. Text highlighted in yellow in top-$k$ SQL indicates tables unnecessary for answering the question. 
% \textbf{Retrieved Table Schema} denotes the schema information for tables retrieved by ATR and top-$k$.
}
\label{tab: case study 2: small k}
\end{table*}

==> tables/data_statistics.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{width=1\columnwidth}
\begin{tabular}{rcccc}
\hline
\multicolumn{1}{l}{\textbf{Dataset}}    & \textbf{\#Q} & \textbf{\#DB} & \textbf{\#T} & \textbf{Min/Max} \\ \hline
\multicolumn{1}{l}{\textbf{Spider}}     &                    &               &  &                \\
Train                          & 6,989              & 140           & 737  &1 / 5              \\
Eval                           & 1,034              & 20            & 81   &1 / 4            \\ \hline
\multicolumn{1}{l}{\textbf{BIRD}}       &                    &               &       &           \\
Train                          & 9,198              & 69            & 522  &1 / 4            \\
Eval                           & 1,534              & 11            & 75   &1 / 4            \\ \hline
\multicolumn{1}{l}{\textbf{Spider 2.0}} &                    &               &  &                \\
Eval                           & 435                & 155           & 6,321 &1 / 366           \\ \hline     
\end{tabular}
\end{adjustbox}
\caption{Data statistics. Number of queries (\#Q), databases (\#DB), tables (\#T), and required tables (Min/Max). Evaluations on Spider and BIRD use development sets.}
\label{tab:datasets}
\end{table}

==> tables/end-to-end_performance.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
 &  & \multicolumn{3}{c}{\textbf{Spider}} & \multicolumn{3}{c}{\textbf{BIRD}} & \multicolumn{3}{c}{\textbf{Spider 2.0}} \\ \cline{3-11} 
 & \textit{k} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gemma\\ (4B/27B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gemma\\ (4B/27B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama\\ (8B/70B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Qwen\\ (7B/32B)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gemma\\ (4B/27B)\end{tabular}} \\ \hline
\multicolumn{11}{l}{\textit{\textbf{Encoder-based}}} \\ \hline
Contriever & 3 & 54.6 / 64.8 & 65.4 / 66.3 & 58.0 / 67.4 & 21.7 / 40.4 & 35.4 / 46.0 & 21.2 / 38.9 & \underline{1.1} / 3.4 & 0.5 / 3.9 & 0.2 / 2.5 \\
 & 5 & 53.3 / 65.0 & 65.7 / 68.6 & 58.3 / 67.7 & 22.4 / 44.5 & 37.0 / 49.8 & 24.1 / 39.7 & \underline{1.1} / 3.2 & 1.4 / 3.7 & 0.7 / 3.2 \\
 & 10 & 54.6 / 67.1 & 66.0 / 70.1 & \underline{60.3} / 67.6 & 24.3 / 47.4 & 39.1 / 53.0 & 25.6 / 43.2 & \underline{1.1} / 3.5 & 0.9 / 4.1 & 0.2 / 3.4 \\
UAE & 3 & 55.7 / 65.0 & 63.6 / 68.0 & 52.5 / 68.1 & 22.6 / 40.7 & 35.1 / 45.4 & 20.1 / 38.8 & 0.7 / 3.5 & 1.1 / 3.4 & 0.5 / 3.4 \\
 & 5 & 54.9 / 66.1 & 66.0 / 69.6 & 52.8 / 70.2 & 23.9 / 45.0 & 37.8 / 49.5 & 22.0 / 43.5 & 0.9 / 3.9 & 1.1 / 3.4 & \underline{0.9} / 4.1 \\
 & 10 & 54.7 / 67.3 & 66.1 / 70.6 & 54.1 / 69.2 & 26.0 / 47.9 & 40.4 / 52.2 & 22.2 / 46.8 & 1.4 / 4.1 & 1.4 / 3.4 & 0.5 / 3.9 \\ \hline
\multicolumn{11}{l}{\textit{\textbf{LLM-based}}} \\ \hline
RankZephyr & 3 & 53.3 / 64.8 & 63.1 / 66.6 & 54.2 / 69.4 & 22.4 / 40.7 & 34.5 / 45.8 & 21.7 / 43.2 & \underline{1.1} / 3.2 & 1.4 / 4.1 & 0.2 / 2.5 \\
 & 5 & 54.8 / 65.9 & 65.4 / 67.2 & 58.2 / 70.2 & 23.0 / 45.0 & 38.1 / 46.2 & 23.2 / 45.5 & 0.9 / 3.0 & 1.1 / 4.1 & 0.7 / 3.0 \\
 & 10 & 57.5 / 67.0 & 66.4 / 67.3 & 59.0 / 70.7 & 25.4 / 47.5 & 39.3 / 49.5 & 24.0 / 46.2 & \underline{1.1} / 3.4 & 1.4 / 3.4 & 0.5 / 4.4 \\
Murre & 3 & 51.2 / 65.3 & 63.4 / 64.6 & 53.6 / 69.3 & 21.8 / 44.5 & 34.2 / 44.2 & 20.9 / 42.8 & 0.9 / 4.1 & 1.4 / 3.2 & \underline{0.9} / 4.1 \\
 & 5 & 53.7 / 65.6 & 64.1 / 65.8 & 54.1 / 70.5 & 22.6 / 44.8 & 37.5 / 45.4 & 20.7 / 44.5 & 0.9 / 3.0 & 1.4 / 3.7 & \underline{0.9} / 3.0 \\
 & 10 & 54.5 / 65.9 & 65.3 / 68.0 & 55.0 / 70.2 & 25.3 / 46.4 & 39.4 / 48.4 & 21.2 / \underline{47.0} & 0.7 / 4.1 & 1.4 / 4.4 & 0.7 / \underline{4.6} \\ \hline
\multicolumn{11}{l}{\textit{\textbf{Reranker-based}}} \\ \hline
JAR (w. Contriever) & 3 & 53.9 / 65.9 & 66.6 / 68.8 & 54.8 / 69.1 & 25.4 / 45.3 & 40.1 / 49.7 & 23.9 / 44.4 & 0.7 / 3.7 & 0.9 / 4.1 & 0.5 / 3.0 \\
 & 5 & 54.8 / 66.6 & 67.5 / 69.7 & 59.4 / 67.8 & 26.8 / 46.4 & 43.4 / 52.0 & \underline{27.4} / 43.2 & \underline{1.1} / 3.9 & 0.7 / 3.7 & \underline{0.9} / 3.2 \\
 & 10 & 56.0 / 66.8 & 66.6 / 69.2 & 59.5 / 67.7 & 26.7 / 47.5 & 43.0 / 53.0 & 24.8 / 44.9 & 0.9 / 3.0 & 1.4 / 4.4 & 0.5 / 4.1 \\
JAR (w. UAE)  & 3 & 54.6 / 67.2 & 66.7 / 66.8 & 55.1 / 69.2 & 24.8 / 44.7 & 38.7 / 44.9 & 22.6 / 44.3 & 0.9 / 3.9 & \underline{1.6} / 4.4 & 0.5 / 2.8 \\
 & 5 & 56.0 / 67.4 & 67.0 / 69.7 & 55.3 / 70.2 & 25.3 / 45.4 & 39.2 / 48.4 & 23.1 / 44.7 & 0.9 / 4.1 & 1.4 / 4.1 & \underline{0.9} / 4.4 \\
 & 10 & 55.6 / 66.9 & 64.6 / 67.7 & 56.6 / \underline{70.8} & 26.6 / 46.9 & 41.3 / 52.2 & 24.2 / 46.6 & 0.9 / 3.0 & \underline{1.6} / 3.7 & \underline{0.9} / 3.2 \\ \hline
\multicolumn{11}{l}{\textit{\textbf{Ours}}} \\ \hline
ATR (w. Contriever) &  & \underline{58.7} / \underline{67.8} & \underline{69.7} / \textbf{71.5} & \textbf{60.7} / 67.8 & \underline{28.6} / \textbf{49.9} & \textbf{45.0} / \underline{53.3} & \textbf{28.8} / 45.1 & \underline{1.1} / \underline{4.4} & 1.4 / \textbf{5.7} & \textbf{1.1} / \textbf{4.8} \\
ATR (w. UAE) &  & \textbf{59.8} / \textbf{68.2} & \textbf{69.8} / \underline{71.4} & 59.0 / \textbf{71.1} & \textbf{29.0} / \underline{48.7} & \underline{43.8} / \textbf{53.9} & 25.6 / \textbf{49.7} & \textbf{1.6} / \textbf{4.5} & \textbf{2.1} / \underline{4.9} & \textbf{1.1} / \underline{4.6} \\ \hline
\multicolumn{1}{l}{\textit{\textbf{Oracle}}} &  & 66.6 / 70.8 & 75.6 / 75.2 & 66.5 / 71.7 & 31.8 / 53.5 & 50.6 / 58.0 & 32.7 / 50.9 & 4.4 / 7.2 & 3.5 / 7.4 & 1.4 / 7.6 \\ \bottomrule
\end{tabular}%
}
\caption{Text-to-SQL execution accuracy comparison across different table retrieval methods. ATR consistently outperforms baseline retrievers on the Spider, BIRD, and Spider 2.0 datasets.}
\label{tab:end-to-end_performance}
\end{table*}

==> tables/llm_reranker.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lc cccc cccc cccc}
\toprule
\multirow{}{}{} & & \multicolumn{4}{c}{\textbf{Spider}} & \multicolumn{4}{c}{\textbf{BIRD}} & \multicolumn{4}{c}{\textbf{Spider 2.0}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & \textbf{k} & P & R & CR & F1 & P & R & CR & F1 & P & R & CR & F1 \\
\midrule
RankGPT-4o-mini & 3 & 48.2 & 96.8 & 93.5 & 62.1 & \textit{54.5} & 88.0 & 76.2 & 65.6 & 33.2 & 48.5 & 33.8 & 35.2 \\
RankGPT-4o-mini & 5 & 29.9 & 98.9 & 97.9 & 44.5 & 35.0 & 92.7 & 84.6 & 49.7 & 24.6 & 56.1 & 42.1 & 30.5 \\
RankGPT-4o-mini & 10 & 15.1 & 99.3 & 99.0 & 25.5 & 18.7 & 97.5 & 94.6 & 30.9 & 15.3 & 64.0 & 52.2 & 21.9 \\
\midrule
RankGPT-5-mini & 3 & 48.9 & 98.2 & 95.5 & 63.1 & \textbf{57.3} & 91.6 & 81.6 & \textbf{66.3} & \textbf{36.6} & 53.6 & 37.5 & \textbf{39.4} \\
RankGPT-5-mini & 5 & 30.0 & 99.5 & 98.9 & 44.8 & 36.4 & 95.7 & 90.0 & 51.5 & 25.8 & 59.3 & 44.1 & 32.4 \\
RankGPT-5-mini & 10 & 15.1 & \textbf{100.0} & \textbf{100.0} & 25.8 & 18.9 & 98.0 & 96.0 & 31.4 & 15.8 & 66.1 & 54.2 & 22.7 \\
\midrule
RankQwen3-32B & 3 & 48.4 & 97.4 & 94.2 & 62.5 & 53.1 & 88.7 & 76.4 & 65.5 & \textit{33.3} & 48.4 & 32.6 & \textit{35.4} \\
RankQwen3-32B & 5 & 30.1 & 99.5 & 98.9 & 44.8 & 35.8 & 94.6 & 87.6 & 50.8 & 24.3 & 55.5 & 40.0 & 30.2 \\
RankQwen3-32B & 10 & 15.1 & 99.4 & 99.0 & 25.6 & 18.9 & 98.0 & \textit{96.4} & 31.2 & 15.3 & 64.0 & 52.0 & 22.0 \\
\midrule
ATR (w. Contriever) &  & \textbf{69.6} & 99.5 & 99.2 & \textbf{78.3} & 54.0 & \textit{98.2} & 96.0 & \textit{65.8} & 21.9 & \textit{72.4} & \textit{64.4} & 27.8 \\
ATR (w. UAE) &  & \textit{69.3} & \textit{99.6} & \textit{99.4} & \textit{78.1} & 52.8 & \textbf{98.6} & \textbf{97.1} & 65.1 & 19.9 & \textbf{75.4} & \textbf{68.7} & 26.7 \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison with LLM-based retrievers and rerankers. \textbf{Bold} indicates the highest score, and \textit{italic} indicates the second-highest score.}
\label{tab:llm_reranker}
\end{table*}

==> tables/main_table.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc}
\toprule
                    &            & \multicolumn{4}{c}{\textbf{Spider}}                           & \multicolumn{4}{c}{\textbf{BIRD}}                             & \multicolumn{4}{c}{\textbf{Spider 2.0}}                       \\ \cline{2-14} 
                    & \textit{k} & \textbf{P}    & \textbf{R}    & \textbf{CR}   & \textbf{F1}   & \textbf{P}    & \textbf{R}    & \textbf{CR}   & \textbf{F1}   & \textbf{P}    & \textbf{R}    & \textbf{CR}   & \textbf{F1}   \\ \hline
\multicolumn{14}{l}{\textit{\textbf{Encoder-based}}}                                                                                                                                                                             \\ \hline
Contriever          & 3          & 46.5          & 94.0          & 89.2          & 60.1          & 45.6          & 72.9          & 55.1          & 54.6          & 24.7          & 37.6          & 24.8          & 27.4          \\
                    & 5          & 29.3          & 97.4          & 95.5          & 43.7          & 31.2          & 82.1          & 68.6          & 44.2          & 19.1          & 45.1          & 32.6          & 24.4          \\
                    & 10         & 15.0          & 99.2          & 98.7          & 25.6          & 18.5          & 96.1          & 92.6          & 30.5          & 13.3          & 56.5          & 44.8          & 19.5          \\
UAE                 & 3          & 46.1          & 93.0          & 88.0          & 59.5          & 48.2          & 79.0          & 63.5          & 58.3          & 27.1          & 40.6          & 27.6          & 29.7          \\
                    & 5          & 29.5          & 97.8          & 96.4          & 44.1          & 32.7          & 87.2          & 77.3          & 46.5          & 20.7          & 48.5          & 34.9          & 26.3          \\
                    & 10         & 15.0          & 99.4          & 99.0          & 25.6          & 18.7          & 97.6          & 95.1          & 30.9          & 14.2          & 60.7          & 49.0          & 20.7          \\ \hline
\multicolumn{14}{l}{\textit{\textbf{LLM-based}}}                                                                                                                                                                                 \\ \hline
RankZephyr          & 3          & 47.7          & 95.9          & 92.8          & 61.5          & 47.9          & 76.6          & 60.4          & 57.3          & 26.0          & 39.3          & 26.4          & 28.7          \\
                    & 5          & 29.5          & 98.2          & 96.9          & 44.1          & 32.1          & 84.4          & 72.4          & 45.5          & 19.7          & 46.7          & 33.8          & 25.2          \\
                    & 10         & 15.1          & \underline{99.5}    & \underline{99.2}    & 25.7          & 18.5          & 96.5          & 93.1          & 30.6          & 13.6          & 57.3          & 45.5          & 19.8          \\
Murre     & 3          & 40.5          & 82.9          & 73.8          & 52.5          & 44.6          & 72.5          & 54.6          & 53.7          & 28.1          & 42.3          & 29.4          & \underline{31.0}    \\
                    & 5          & 26.9          & 90.3          & 85.5          & 40.3          & 30.1          & 80.5          & 66.4          & 42.8          & 21.8          & 51.1          & 36.8          & 28.0          \\
                    & 10         & 14.6          & 96.8          & 95.1          & 24.8          & 16.7          & 88.2          & 78.3          & 27.6          & 14.8          & 61.9          & 48.5          & 21.5          \\ \hline
\multicolumn{14}{l}{\textit{\textbf{Reranker-based}}}                                                                                                                                                                            \\ \hline
% BGE-M3 + Contriever & 3          & 46.0          & 93.1          & 87.7          & 59.5          & 39.4          & 64.7          & 44.4          & 47.6          & 24.7          & 33.4          & 21.2          & 24.7          \\
%                     & 5          & 28.9          & 96.7          & 93.7          & 43.3          & 29.5          & 78.9          & 64.2          & 41.9          & 19.2          & 40.2          & 26.7          & 22.1          \\
%                     & 10         & 14.9          & 99.1          & 98.1          & 25.4          & 17.4          & 91.3          & 83.6          & 28.8          & 14.2          & 52.6          & 40.5          & 18.3          \\
% BGE-M3 + UAE        & 3          & 45.7          & 92.5          & 87.1          & 59.1          & 37.4          & 61.2          & 40.7          & 45.2          & 24.2          & 33.9          & 21.6          & 24.9          \\
%                     & 5          & 28.8          & 96.5          & 93.2          & 43.2          & 28.3          & 76.1          & 61.3          & 40.4          & 19.5          & 43.4          & 29.4          & 23.3          \\
%                     & 10         & 14.9          & 98.8          & 97.6          & 25.4          & 17.2          & 90.5          & 82.2          & 28.4          & 14.0          & 54.1          & 40.7          & 18.5          \\
JAR (w. Contriever)    & 3          & 48.1          & 96.5          & 93.6          & 62.0          & \textbf{54.4} & 87.4          & 76.3          & 65.0          & \textbf{29.4} & 42.3          & 26.9          & \textbf{31.6} \\
                    & 5          & 29.7          & 98.5          & 97.2          & 44.3          & 35.1          & 92.5          & 85.9          & 49.7          & 21.9          & 48.6          & 34.0          & 27.0          \\
                    & 10         & 15.1          & \underline{99.5}    & \underline{99.2}    & 25.7          & 18.8          & 97.6          & \underline{96.0}    & 31.0          & 14.0          & 55.1          & 41.4          & 19.5          \\
JAR (w. UAE)           & 3          & 48.4          & 96.5          & 94.1          & 62.3          & 53.6          & 86.3          & 74.8          & 64.4          & \underline{29.1}    & 41.6          & 27.1          & 30.8          \\
                    & 5          & 29.9          & 99.1          & 98.5          & 44.7          & 34.4          & 91.1          & 82.9          & 48.9          & 21.8          & 47.9          & 33.8          & 26.5          \\
                    & 10         & 15.1          & \underline{99.5}    & \underline{99.2}    & 25.7          & 18.7          & 97.2          & 95.2          & 30.9          & 14.3          & 56.4          & 43.9          & 19.7          \\ \bottomrule
\multicolumn{14}{l}{\textit{\textbf{Ours}}}                                                                                                                                                                                      \\ \hline
ATR (w. Contriever)    &            & \textbf{69.6} & \underline{99.5}    & \underline{99.2}    & \textbf{78.3} & \underline{54.0}    & \underline{98.2}    & \underline{96.0}    & \textbf{65.8} & 21.9          & \underline{72.4}    & \underline{64.4}    & 27.8          \\
ATR (w. UAE)           &            & \underline{69.3}    & \textbf{99.6} & \textbf{99.4} & \underline{78.1}    & 52.8          & \textbf{98.6} & \textbf{97.1} & \underline{65.1}    & 19.9          & \textbf{75.4} & \textbf{68.7} & 26.7          \\ \bottomrule
\end{tabular}%
}
\caption{Retrieval performance comparison with baseline methods, evaluated using Precision (P), Recall (R), Complete Recall (CR), and F1 scores (F1). 
We use SGPT-5.8B as the backbone model for Murre.
ATR consistently outperforms all baselines across datasets. The best and second-best scores for each metric are highlighted in \textbf{bold} and \underline{underlined}, respectively.}
\label{Experiments:Main Result}
\end{table*}

==> tables/memory_profiling.tex <==
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll ccc}
\toprule
\textbf{Dataset} & \textbf{Metric} & \textbf{Sliding Window (Ours)} & \textbf{No Sliding Window} & \textbf{Reduction} \\
\midrule
\multirow{}{}{Spider} & Avg Peak & 30.62 MB & 63.98 MB & 52.1\% \\
 & Max Peak & 44.01 MB & 80.67 MB & 45.4\% \\
\midrule
\multirow{}{}{BIRD} & Avg Peak & 51.76 MB & 93.32 MB & 44.5\% \\
 & Max Peak & 94.31 MB & 145.13 MB & 35.0\% \\
\midrule
\multirow{}{}{Spider 2.0} & Avg Peak & 66.52 MB & 340.57 MB & 80.5\% \\
 & Max Peak & 284.44 MB & 1027.88 MB & 72.3\% \\
\bottomrule
\end{tabular}
}
\caption{GPU memory consumption profiling on the test sets. Avg Peak refers to the average maximum memory allocated per sample, and Max Peak denotes the single highest memory spike observed during inference.}
\label{tab:memory_profiling}
\end{table}

==> tables/proprietary_embed.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1.3mm} 
\begin{adjustbox}{width=1\columnwidth}
\begin{tabular}{lccccccc}
\toprule
                &      & \multicolumn{2}{c}{\textbf{Spider}}                                                     & \multicolumn{2}{c}{\textbf{BIRD}}                                                         & \multicolumn{2}{c}{\textbf{Spider 2.0}}                                                   \\ 
                \cmidrule{3-8}
                &   $k$   & \textbf{R}    & \textbf{\begin{tabular}[c]{@{}c@{}}CR\end{tabular}} & \textbf{R}      & \textbf{\begin{tabular}[c]{@{}c@{}}CR\end{tabular}} & \textbf{R}      & \textbf{\begin{tabular}[c]{@{}c@{}}CR\end{tabular}} \\ \toprule
\textbf{OpenAI} & 3  & 96.8              & 93.5                                                              & 85.8                & 72.1                                                              & 40.7                & 28.2                                                              \\
\textbf{}       & 5  & \underline{99.7}              & 99.4                                                              & 92.8                & 85.5                                                              & 50.0                & 36.7                                                              \\
\textbf{}       & 10 & { \textbf{100}} & { \textbf{100}}                                                 & \underline{ 98.4} & \underline{ 96.7}                                               & \underline{ 62.8}          & \underline{ 49.8}                                                        \\ \midrule
\textbf{ATR (Ours)}   &      & 99.6        & \underline{ 99.6}                                                        & {\textbf{99.5}}          & {\textbf{99.2}}                                                        & {\textbf{79.5}} & {\textbf{70.2}}                                               \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Evaluation of retrieval performance comparing ATR and a proprietary embedding model. OpenAI indicates text-embedding-3-large.}
\label{tab:proprietary embed}
\end{table}

==> tables/sliding_analysis.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{cccccccccc}
\hline
                                                                               & \multicolumn{3}{c}{\textbf{Spider}} & \multicolumn{3}{c}{\textbf{BIRD}} & \multicolumn{3}{c}{\textbf{Spider 2.0}} \\ \hline
\textbf{W, R} & 50, N/A     & 20, 15     & 10, 6    & 50, N/A    & 20, 15     & 10,6    & 50, N/A       & 10, 5      & 6, 4       \\ \hline
\textbf{Time}                                                           & 0.12        & 0.14       & 0.17     & 0.18       & 0.21       & 0.26    & 0.60          & 0.41       & 0.45       \\
\textbf{Length}                                                                  & 1164.4      & 471.7      & 237.5    & 1592.7     & 617.9      & 324.0   & 3982.8        & 846.2      & 532.8      \\
\textbf{\# Inference}                                                          & 1           & 7          & 11       & 1          & 7    & 11      & 1             & 9          & 23         \\ \hline
\end{tabular}
\caption{Analysis of sliding window hyper-parameters $W$ and $R$, where $W$ denotes the window size and $R$ is the retention size. The metrics include average inference time in seconds (Time), average input token length (Length), and number of inferences (\# Inference).}
\label{tab:sliding analysis}
\end{table*}
